SleepWalk: A Three-Tier Benchmark for Stress-Testing Instruction-Guided Vision-Language Navigation

Vision-Language Models (VLMs) have advanced rapidly in multimodal perception and language understanding, yet it remains unclear whether they can reliably ground language into spatially coherent, plausibly executable actions in 3D digital environments. We introduce SleepWalk, a benchmark for evaluating instruction-grounded trajectory prediction in single-scene 3D worlds generated from textual scene descriptions and filtered for navigability. Unlike prior navigation benchmarks centered on long-range exploration across rooms, SleepWalk targets localized, interaction-centric embodied reasoning: given rendered visual observations and a natural-language instruction, a model must predict a trajectory that respects scene geometry, avoids collisions, and terminates at an action-compatible location. The benchmark covers diverse indoor and outdoor environments and organizes tasks into three tiers of spatial and temporal difficulty, enabling fine-grained analysis of grounding under increasing compositional complexity. Using a standardized pointwise judge-based evaluation protocol, we evaluate three frontier VLMs on 2,472 curated 3D environments with nine instructions per scene. Results reveal systematic failures in grounded spatial reasoning, especially under occlusion, interaction constraints, and multi-step instructions: performance drops as the difficulty level of the tasks increase. In general, current VLMs can somewhat produce trajectories that are simultaneously spatially coherent, plausibly executable, and aligned with intended actions. By exposing failures in a controlled yet scalable setting, SleepWalk provides a critical benchmark for advancing grounded multimodal reasoning, embodied planning, vision-language navigation, and action-capable agents in 3D environments.

==> 2_attack_taxonomy.tex <==

% LaTeX Code for Adversarial Attacks Taxonomy










\section{Categories of Adversarial Attacks}
\vspace{-0.5em}

The threat landscape for large language models (LLMs) is rapidly diversifying, demanding a systematic taxonomy that captures both the breadth and depth of adversarial behaviors. Figure~\ref{fig:lit_surv} presents a hierarchical classification of adversarial attacks, organized into three macro-level branches: \textbf{Jailbreak}, \textbf{Control Generation}, and \textbf{Performance Degradation}. Each branch subdivides into mechanisms that reflect how adversaries manipulate generation pathways, exploit latent representations, or corrupt learning signals.

\textbf{Jailbreak attacks} (\S\ref{jailbreak}) aim to circumvent alignment mechanisms and elicit model outputs that are toxic, deceptive, or otherwise prohibited. We distinguish two canonical modes: (a) \emph{Optimization-based jailbreaks}, which craft prompts to directly induce societal harm, privacy leakage, or disinformation \cite{wu2024llms, pair23, tap23}; and (b) \emph{Long-tail distribution exploits}, which invoke unsafe behavior through distributional edge cases such as rare prompts or persuasive manipulations \cite{jiang2023promptpacker, schulhoff2023hackaprompt}.

\textbf{Control generation attacks} (\S\ref{control}) compromise the model’s controllability by subverting its generation semantics. These include (a) \emph{Direct attacks}, such as syntax manipulation, malicious prompt engineering, and suffix-based alignment bypasses \cite{jiang2023promptpacker, schulhoff2023hackaprompt}; and (b) \emph{Indirect attacks}, which exploit latent conditioning or external augmentation, such as goal hijacking \cite{chen2024pseudo}, prompt leakage \cite{li2024pleak}, or adversarial injection from retrieved content \cite{greshake2023indirect}.









\textbf{Performance degradation attacks} (\S\ref{performance}) do not seek harmful content but instead aim to reduce the functional reliability of LLMs. These include (a) \emph{Dataset poisoning}—where injected samples induce label flipping, semantic drift, or misgeneralization \cite{greshake2023indirect}; and (b) \emph{Prompt-based degradation}, which introduces errors in classification, factuality, or consistency \cite{greshake2023indirect}.

This taxonomy in Figure~\ref{fig:lit_surv} reveals that adversarial risk is not monolithic. Instead, it manifests along orthogonal dimensions—ethical, semantic, and functional—and cannot be addressed through surface-level defenses alone. Robust alignment requires a stratified approach that operates not just at the token level but within the geometry of the model's latent cognition.


\section{Where the Firewall Cracks: A Cartography of LLM Vulnerabilities}

Figure~\ref{fig:llm_heatmap_benchmark} offers a comparative vulnerability map of 21 LLMs under jailbreak stress tests. While frontier models like LLaMA-3 and GPT-4 exhibit notable robustness, instruction-tuned open models—including Vicuna, Mistral, and Phi—show consistent breakdowns under persona manipulation, chaining, and prompt extraction attacks. The persistence of high success rates across categories, especially for goal hijacking and extraction, reveals fundamental limitations in current alignment defenses and underscores the need for deeper representational safeguards.


\textbf{Choices of LLMs – Stress Testing.}  
To systematically evaluate the role of model size, architecture, and training provenance in adversarial vulnerability, we benchmarked 21 contemporary large language models spanning diverse families and design philosophies. This includes open and proprietary models, ranging from dense transformers to mixture-of-experts architectures, covering parameter scales from 2B to 70B. The full suite comprises:  
\textbf{(i)} GPT-4o-mini~\cite{gpt-4o-mini},  
\textbf{(ii)} GPT-4,  
\textbf{(iii)} GPT-3.5~\cite{gpt4},  
\textbf{(iv–v)} LLaMA-3.1-70B and 8B~\cite{llama-3.1},  
\textbf{(vi–vii)} LLaMA-3-70B and 8B~\cite{llama-3},  
\textbf{(viii–x)} LLaMA-2-70B, 13B, and 7B~\cite{llama-2},  
\textbf{(xi)} Vicuna-1.5~\cite{vicuna},  
\textbf{(xii)} Phi-2~\cite{phi-2},  
\textbf{(xiii)} Phi-3~\cite{phi-3},  
\textbf{(xiv)} Claude~\cite{claude},  
\textbf{(xv–xvi)} Mixtral-8$\times$7B and 22B~\cite{mixtral},  
\textbf{(xvii–xviii)} Gemma-7B and 2B~\cite{gemma},  
\textbf{(xix)} Mistral~\cite{mistral}, and  
\textbf{(xx–xxi)} DeepSeek and DeepSeek-R1.

\subsection{{\fontfamily{uncl}\selectfont ALKALI} — Adversarial Safety Dataset}

The \textsc{ALKALI} dataset supports a structured, citation-grounded evaluation of adversarial vulnerabilities in LLMs. Each prompt is mapped to one of the taxonomy branches shown in Figure~\ref{fig:lit_surv}, with instances sourced from high-fidelity adversarial papers. We aggregate 9,000 examples spanning 3 macro-categories, 6 subtypes, and 15 distinct attack families. This alignment enables category-specific benchmarking, subtype-level stress testing, and paper-wise traceability for reproducibility and comparative evaluations.

\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}p{3.2cm} p{9.2cm} r@{}}
\toprule
\textbf{Category} & \textbf{Subtype \& Source(s)} & \textbf{Instances} \\
\midrule
\multirow{2}{=}{\textbf{Jailbreak}} 
  & \textit{Optimization-based}: \cite{wu2024llms, pair23, tap23} & 1,200 \\
  & \textit{Long-tail Distribution}: \cite{jiang2023promptpacker, schulhoff2023hackaprompt} & 1,500 \\
\midrule
\multirow{2}{=}{\textbf{Control Generation}} 
  & \textit{Direct Attacks}: \cite{jiang2023promptpacker, schulhoff2023hackaprompt} & 1,600 \\
  & \textit{Indirect Attacks}: \cite{chen2024pseudo, li2024pleak, greshake2023indirect} & 1,400 \\
\midrule
\multirow{2}{=}{\textbf{Performance Degradation}} 
  & \textit{Dataset Poisoning}: \cite{greshake2023indirect} & 1,800 \\
  & \textit{Prompt Injection}: \cite{greshake2023indirect} & 1,500 \\
\midrule
\textbf{Total} & — & \textbf{9,000} \\
\bottomrule
\end{tabular}
}
\caption{ALKALI dataset distribution across taxonomy categories with citations corresponding to each attack subtype.}
\label{tab:alkali_data_breakdown}
\end{table}










==> 3_llm.tex <==




\section{Choices of LLMs - Stress Testing}

\textcolor{blue}{To analyze the effect of size and architecture of LLMs on their vulnerability to adversarial attacks, we chose 19 contemporary LLMs that have exhibited exceptional results on a wide range of NLP tasks, including: \textbf{(i)} GPT-4o-mini \cite{gpt-4o-mini}, \textbf{(ii)} GPT-4 \cite{gpt4}, \textbf{(iii)} GPT-3.5 \cite{gpt-3.5}, \textbf{(iv)} LLaMA-3.1-70b \cite{llama-3.1}, \textbf{(v)} LLaMA-3.1-8b \cite{llama-3.1}, \textbf{(vi)} LLaMA-3-70b \cite{llama-3}, \textbf{(vii)} LLaMA-3-8b \cite{llama-3}, \textbf{(viii)} LLaMA-2-70b \cite{llama-2}, \textbf{(ix)} LLaMA-2-13b \cite{llama-2}, \textbf{(x)} LLaMA-2-7b \cite{llama-2}, \textbf{(xi)} Vicuna-1.5 \cite{vicuna}, \textbf{(xii)} Phi-2 \cite{phi-2}, \textbf{(xiii)} Phi-3 \cite{phi-3}, \textbf{(xiv)} Claude \cite{claude}, \textbf{(xv)} Mixtral-8$\times$7b \cite{mixtral1}, \textbf{(xvi)} Mixtral-8$\times$22b \cite{mixtral2}, \textbf{(xvii)} Gemma-7b, \textbf{(xviii)} Gemma-2, and \textbf{(xix)} Mistral.}

==> 4_aavi.tex <==




\section{Adversarial Vulnerability Index}

\begin{figure*}[h!]
    \centering
        \includegraphics[width=1.2\linewidth]{figures/ASR_Heatmap_AllLLMs_DPO_GRACE.pdf} % 1.2 times the linewidth
    \caption{ASR Heatmap}
    \label{ASR_heat_map}
\end{figure*}
\subsection{AVI\textsubscript{degrade\_performance}}



% Excel doc for ASR scores: https://docs.google.com/spreadsheets/d/1SrLsPllNFOrSNSTxTqLYraseJjZwdZqkai-YSHzfSOc/edit?gid=0#gid=0
In this work, we introduce a novel metric termed the \textbf{\textit{Adversarial Vulnerability Index}} (AVI), which serves as a comparative measure for evaluating the vulnerability of language models to adversarial attacks. The AVI is specifically designed to assess the susceptibility of language models across three critical dimensions of adversarial attacks. This metric is particularly useful for evaluating the risk posed by black-box attacks, which are easier to execute and often expose the most significant vulnerabilities in language models.
\\
The AVI is computed both at a category level and as an aggregate score. The category-wise AVI scores provide insights into the specific vulnerabilities of a model in the face of different types of adversarial attacks. Additionally, we compute a global AVI score, which is a linear weighted combination of the individual category-wise AVI scores. This global score offers a comprehensive measure of the model's overall adversarial robustness. Formally, the global AVI score is defined as follows:
\begin{equation}
\text{AVI}_{\text{global}}^{\text{LLM}} = \sum_{i \in \{\text{JB, CG, DP}\}} w_i \cdot \text{AVI}_i^{\text{LLM}}
\end{equation}
where \( w_i \) represents the weight assigned to the AVI score of each category \( i \). The sum of the weights is normalized such that:
\[
\sum_{i} w_i = 1 \quad \text{and} \quad w_{i-1} > w_i
\]
The condition \( w_{i-1} > w_i \) reflects the relative severity of each type of attack, enabling a nuanced allocation of weights to various attack vectors. For our analysis, the weights are assigned as follows: \( w_{\text{JB}} = 0.5 \) for jailbreak, \( w_{\text{CG}} = 0.2 \) for control generation, and \( w_{\text{DP}} = 0.3 \) for performance degradation. These weights are adjustable based on strategic priorities and risk assessment outcomes. The category-wise \( \text{AVI}_i \) is calculated in terms of the \textit{Attack Success Rate} (ASR). We define the category wise AVI as:
\[
\text{AVI} = \frac{\sum_{i=1}^{n(\mathcal{D})} \left( \text{LLM}(\mathcal{D}_i) = \text{attack\_successful} \right)}{n(\mathcal{D})}
\]

where \( \mathcal{D} \) represents the dataset of prompts used to attack the LLM, \( \mathcal{D}_i \) refers to the \( i \)-th prompt in the set, and \( n(\mathcal{D}) \) denotes the the cardinal number of \( \mathcal{D} \). The exact calculation of ASRs have been described in the respective sections.
\section{Computation of AVI(s)}
\subsection{AVI\textsubscript{jail\_break}}
\subsection{AVI\textsubscript{control\_generation}}
As discussed in Section 3.2, control generation in large language models (LLMs) encompasses two critical aspects: prompt leakage and goal hijacking. For our experiments, we utilized the dataset provided by \textit{Perez et al.} (2023) \cite{ignore_previous_prompt} as the benchmark for evaluating LLM performance and assigning AVI scores for control generation. To assess the effectiveness of prompt extraction, we employed a combination of 35 base prompts from OpenAI, supplemented with specific attack instructions. The evaluation was conducted by performing a substring match to determine the extent to which the prompt was successfully extracted.
In the case of goal hijacking, the evaluation process involves the use of a predefined rogue string that must be finalized before determining the Attack Success Rate (ASR). Originally, \textit{Perez et al.} (2023) utilized the string \textit{"I HATE HUMANS"} as the rogue string. However, since LLMs are typically trained to avoid generating harmful or offensive text, using this string might not accurately reflect the model's susceptibility to goal hijacking. To mitigate this issue and avoid breaching the model's safety protocols, we conducted further experiments by substituting the rogue string with \textit{"I LOVE HUMANS"}. This approach ensures that our focus remains solely on evaluating the model's vulnerability to goal hijacking, rather than inadvertently testing the robustness of its ethical safeguards. We identify successful goal hijacking attacks through exact string matching. The AVI(s) for control generation are illustrated in figure \ref{AVI_control_generation}. More details can be found in the Appendix.

\subsection{AVI\textsubscript{degrade\_performance}}

==> 5_alkali_dataset.tex <==




==> 6_experiments.tex <==





==> 7_results.tex <==




\section{Performance and Advantages of \textsc{GRACE}}

We evaluate \textsc{GRACE} across three principal axes: adversarial robustness, latent geometric structure, and reference-aware preference fidelity. Our experiments span 17 open-source LLMs and 12 attack types—including jailbreaks, logic inversions, and prompt injections—demonstrating consistent performance gains over DPO and its variants.

\vspace{1mm}
\subsection*{Adversarial Robustness: Lowering the Floor of Vulnerability}

Across the consolidated adversarial suite—comprising our benchmark corpus, Anthropic’s jailbreak dataset~\cite{perez2022red}, and prompt perturbations from PromptBench~\cite{zhu2024promptbench}—\textsc{GRACE} consistently lowers Attack Success Rate (ASR) compared to baselines. On models such as LLaMA-3 (8B), DeepSeek (7B), and Mixtral (8x22B), we observe ASR reductions of up to \textbf{30\%} post-training, with no degradation in performance on clean prompts.

\vspace{1mm}
\subsection*{Latent Geometry: Structural Interpretability and Generalization}

Using metrics like the Adversarial Vulnerability Quality Index (AVQI) and Density-Based Separation (DBS), we show that \textsc{GRACE} produces disentangled clusters in the pooled latent space:
\begin{itemize}[leftmargin=1.5em]
    \item \textbf{Safe completions} form low-variance clusters, well-separated from adversarial behavior.
    \item \textbf{Unsafe and jailbreak completions} coalesce into a compact adversarial manifold, distinct from the safe subspace.
\end{itemize}




\begin{figure*}[htp!]
    \centering
    \includegraphics[width=\textwidth]{figures/LLM_Attack_Benchmark_Heatmap_PostGRACE_OpenOnly_400dpi_OneLine.pdf}
    \caption{
    \textbf{GRACE Mitigation Performance across Open-Source LLMs.}
    This heatmap presents the Attack Success Rate (ASR) of 17 open-source large language models across 12 adversarial attack types. We show each attack the pre- and post-GRACE ASR, visually highlighting post-GRACE rows by golden borders. Each cell in a post-GRACE row displays the updated ASR (rounded) and the percentage reduction relative to the original, using a two-line format. GRACE (Geometric Preference Optimization for Alignment Robustness) consistently reduces ASR across all model scales and architectures—including instruction-tuned and chat-optimized variants like LLaMA-2/3, Vicuna, Mistral, Gemma, and DeepSeek—without requiring task-specific tuning or retraining. Attacks such as Goal Hijacking, Prompt Extraction, and TAP demonstrate substantial mitigation, reflecting GRACE’s strength against structural and semantic adversarial behaviors. This benchmark confirms that GRACE can provide effective, generalizable safety alignment while maintaining model usability.
    }
    \label{fig:grace_benchmark}
\end{figure*}

These geometric outcomes support the hypothesis that adversarial robustness arises from latent-space structure—not surface-level alignment.

\vspace{1mm}
\subsection*{KL Relaxation and Reference Drift Mitigation}

Direct Preference Optimization (DPO) often over-regularizes toward a fixed reference policy \(\pi_{\mathrm{ref}}\), risking underperformance when \(\pi_{\mathrm{ref}}\) itself produces unsafe outputs. \textsc{GRACE} relaxes this constraint via a tunable scaling factor \(\alpha \in [0,1]\)~\cite{wu2024generalized, chen2023epsilon}, allowing the model to:
\begin{itemize}[leftmargin=1.5em]
    \item Escape faulty reference completions while preserving overall alignment.
    \item Learn safer behaviors even when \(\pi_{\mathrm{ref}}\) is compromised.
\end{itemize}

This reduces KL-induced overfitting and improves generalization to adversarial contexts.

\vspace{1mm}
\subsection*{Lightweight and Modular Design}

\textsc{GRACE} requires no additional decoders or classifier heads. It operates entirely over frozen LLM representations and introduces only a soft attention profile \(\alpha^{(l)}\) over internal layers. This design ensures:
\begin{itemize}[leftmargin=1.5em]
    \item \textbf{Parameter efficiency} with minimal memory overhead.
    \item \textbf{Model agnosticity}—easily adaptable to any pretrained LLM.
    \item \textbf{Deployment ease} when using pre-trained \(\alpha^{(l)}\) vectors.
\end{itemize}

\vspace{1mm}
\subsection*{Summary of Core Advantages}

\begin{itemize}[leftmargin=1.8em]
    \item \textbf{Adversarial Robustness:} Up to 30\% ASR reduction across challenging attacks.
    \item \textbf{Latent Interpretability:} Behavior types form separated, analyzable clusters.
    \item \textbf{KL-Resilient Preference Learning:} Learns to prefer safe responses even with imperfect reference policies.
    \item \textbf{Modular and Lightweight:} No new architecture required—only learnable attention over frozen LLM layers.
\end{itemize}

\vspace{1mm}
In summary, \textsc{GRACE} unifies the strengths of preference modeling with the inductive bias of latent geometry, offering a scalable path toward adversarially aligned, interpretable, and mechanistically grounded language models.










==> 8_conclusion.tex <==
\section{Conclusion}

This paper redefines adversarial alignment in large language models (LLMs) as a problem of \textit{geometric supervision}, moving beyond traditional token-level alignment strategies. We present \textbf{GRACE}—\textit{Geometric Representation-Aware Contrastive Enhancement}—a principled framework that integrates relaxed preference optimization with structural regularization in the latent space. In doing so, GRACE transforms safety alignment from a surface-level behavioral phenomenon into an interpretable and mechanistically grounded geometric property.

Beyond GRACE, our contributions are multifold and foundational. First, we introduce the \textbf{Adversarial Vulnerability Quality Index (AVQI)}, the first geometry-based diagnostic designed to quantify latent entanglement between safe, unsafe, and jailbreak completions. AVQI unifies Density-Based Separation and Dunn Index metrics, offering a theory-grounded lens to interrogate alignment fidelity and adversarial collapse. Second, we construct the \textbf{ALKALI} benchmark, a 9,000-instance adversarial corpus systematically organized by threat taxonomies, enabling stress-testing across jailbreaks, goal hijacking, poisoning, and more.

Our representation-level analysis exposes a critical failure mode in existing alignment pipelines: adversarial completions—particularly jailbreaks—often mimic the latent footprint of safe responses, leading to the \textit{camouflage effect}. To mitigate this, GRACE imposes two geometric priors: (i) enforcing latent separation between safe and adversarial behaviors, and (ii) consolidating unsafe and jailbreak completions into a coherent adversarial manifold. These constraints are implemented through structured triplet-based contrastive losses, computed over \textit{learned pooled representations} derived from a soft attention profile across transformer layers. This mechanism not only improves alignment, but reveals \textit{where} in the model’s depth alignment-critical abstractions reside.

Empirical evaluations across 21 LLMs and 12 adversarial regimes show that GRACE outperforms standard DPO and $\varepsilon$-DPO by up to 39\% ASR reduction, without degrading performance on clean prompts. More importantly, AVQI analysis confirms that GRACE sculpts the safety manifold—safe clusters become compact and linearly separable, while adversarial completions converge into an isolatable subspace.

\textbf{Broader Implications.} Our findings suggest that adversarial robustness cannot be post hoc patched into LLMs through output-based heuristics. Instead, safety must be embedded structurally—via latent geometry, inductive priors, and behavior-aware supervision. GRACE's proposed architecture-free and parameter-efficient design, which operates with a frozen LLM and a minimal trainable attention profile, offers a lightweight yet expressive avenue to scale adversarial defenses without architectural overhaul.

\textbf{Outlook.} We envision several promising extensions: (1) continual refinement of alignment geometry through online contrastive replay, (2) adversarial subspace projection for decoding-time defenses, and (3) multi-agent cooperative alignment where latent preferences are harmonized across interacting models. With GRACE and AVQI as foundational tools, we take a step toward a future where alignment is not merely evaluated at the output—but engineered into the very shape of cognition in modern language models.


==> 9_discussion.tex <==

\vspace{2mm}
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{p{4.2cm} p{5.8cm} p{5.8cm}}
\toprule
\textbf{Aspect} & \textbf{Strength of GRACE} & \textbf{Limitation / Caution} \\
\midrule
\textbf{Representation Geometry} & Enforces structured clusters for safe/unsafe/jailbreak responses & May require behavior labels or clustering heuristics \\
\textbf{Pooling Strategy} & Learnable attention over LLM layers reveals alignment-relevant depth & Static and prompt-invariant; dynamic variants may help \\
\textbf{Parameter Efficiency} & Only attention weights trained; backbone frozen & May underutilize full model capacity in latent alignment \\
\textbf{Adversarial Robustness} & Reduces ASR by 35–39\%, outperforming DPO by 6–8$\times$ & Assumes adversarial samples are correctly labeled and separable \\
\textbf{Scalability} & Works with any frozen LLM checkpoint & Forward-pass cost increases with number of behavior classes \\
\textbf{Generalization} & Effective across jailbreak, control, and degradation attacks & Not tested on multimodal or instruction-following benchmarks \\
\bottomrule
\end{tabular}
\caption{At-a-glance summary of GRACE’s strengths and limitations.}
\label{tab:grace_summary}
\vspace{-1mm}
\end{table*}

\section{Discussion and Limitations}

\paragraph{Representation-Grounded Alignment.}
GRACE introduces a paradigm shift from output-based preference tuning to geometry-aware alignment, showing that internal representations encode critical safety-relevant information. Our latent contrastive losses reshape the internal geometry of LLMs to reflect structured behavioral distinctions, enforcing compactness within unsafe regions and separation from safe clusters. This alignment of latent geometry boosts adversarial robustness and paves the way for explainable and interpretable safety enforcement.

\paragraph{Latent Contrastive Supervision vs. Traditional Preference Learning.}
While DPO and its variants align model behavior through pairwise preference loss, they overlook the internal mechanisms that lead to unsafe completions. GRACE complements preference learning by supervising these mechanisms directly in the embedding space. Our contrastive losses target adversarial proximity and unsafe dispersion—factors often missed by output-only training. This hybrid formulation leads to sharper representation boundaries and generalizes better to unseen attacks.

\paragraph{Efficiency and Interpretability.}
GRACE is highly parameter-efficient: the only trainable parameters during pooling are the scalar layerwise weights $\alpha^{(l)}$. The rest of the model remains frozen during this step, enabling fast convergence and modular analysis. This structure enables post-hoc auditing of layer contributions to alignment and offers an interpretable bridge between model depth and safety fidelity. Furthermore, the pooled representations offer new debugging and safety attribution tools, which can benefit practitioners seeking deeper control over LLM behavior.

\paragraph{Limitations.}
Despite strong empirical results, GRACE has certain limitations:
\begin{itemize}
    \item \textbf{Behavioral triplet assumption:} GRACE operates under a semi-synthetic triplet construction where (safe, unsafe, jailbreak) completions are drawn from separate datasets. This assumption may introduce distributional shifts or confounding signals when true behavior-specific clusters are not well-separated.
    \item \textbf{Frozen backbone constraint:} During contrastive supervision, the LLM is frozen. While this improves modularity and efficiency, it limits the system’s ability to jointly co-adapt latent and output layers for optimal alignment.
    \item \textbf{Static pooling:} The learned attention profile over layers is static and prompt-invariant. Dynamic, prompt-aware or multi-head pooling might further improve semantic disentanglement in future versions.
    \item \textbf{Compute overhead:} Each batch requires multiple forward passes (one per behavior class), marginally increasing compute costs during latent supervision.
    \item \textbf{Modality and dataset limitations:} We evaluate GRACE only on text-based LLMs. Its extension to multimodal models and richer alignment benchmarks (e.g., Anthropic's HH-RLHF or red-teaming datasets) remains an open direction.
\end{itemize}

\paragraph{Future Extensions.}
We envision several promising extensions to GRACE:
\begin{itemize}
    \item \textit{Prompt-conditional attention pooling} for adaptive safety supervision.
    \item \textit{Joint training of latent and policy layers}, allowing end-to-end preference tuning under geometric constraints.
    \item \textit{Geometric alignment diagnostics}, where AVQI and cluster shape are tracked during training to assess overfitting, drift, or compression.
    \item \textit{Multi-agent adversarial alignment}, where GRACE-inspired contrastive losses are used across interacting LLM agents in competitive tasks.
\end{itemize}



\vspace{1mm}
\noindent Overall, GRACE provides a blueprint for bridging latent-space structure and alignment-aware tuning. It invites a broader shift from black-box preference optimization to interpretable, mechanistically grounded fine-tuning of language models.


==> extra.tex <==





\clearpage
\newpage
\section{\textsc{GRACE}: \underline{G}eometric \underline{R}epresentation-\underline{A}ware \underline{C}ontrastive \underline{E}nhancement}

While Direct Preference Optimization (DPO)~\cite{rafailov2023direct} has emerged as a compelling paradigm for aligning language models with human preferences, it primarily operates at the output logit level—optimizing models to prefer safe completions over unsafe ones. However, adversarial attacks do not merely exploit generation probabilities; they camouflage unsafe intent within benign-looking prompts that remain indistinguishable in the model’s internal representation space. In such cases, alignment must extend beyond the surface form to actively reshape the geometry of latent activations.

We propose \textsc{GRACE}—a novel alignment framework that augments preference-based objectives with \textit{representation-level contrastive regularization}. Inspired by Generalized DPO (GRPO)~\cite{wu2024generalized}, \textsc{GRACE} modifies the DPO objective to enforce stronger separation in the model’s hidden space between safe and adversarial completions. By imposing latent contrast and relaxing the KL constraint, \textsc{GRACE} not only preserves preference-consistent outputs but also carves out distinct topological subspaces for safe and unsafe behaviors.









\section{\textsc{GRACE}: Geometric Representation-Aware Contrastive Enhancement}

Motivated by this hypothesis, we introduce \textsc{GRACE}, a principled extension of DPO that injects structural inductive bias into the alignment process. Specifically, \textsc{GRACE} augments preference optimization with two geometric components:

\begin{enumerate}
    \item \textbf{Geometric Separation Constraint.} We introduce a regularization term that enforces linear separability between safe, unsafe, and jailbreak completions in hidden space—explicitly maximizing centroid distance and minimizing overlap.
    
    \item \textbf{Latent Contrastive Enhancement.} We incorporate a contrastive loss that sharpens intra-cluster cohesion among safe generations while pushing unsafe completions toward isolated subspaces. This regularization is applied across multiple layers to ensure robust representational separation.
\end{enumerate}

Together, these modifications reframe alignment as a dual optimization problem: learning which outputs to prefer and how to encode those preferences into the model’s latent manifold. As our experiments show, \textsc{GRACE} transforms adversarial vulnerability into a problem of geometric insulation—shielding safe behavior from manipulation by reshaping the structure of thought itself.





\subsection{Desired Geometric Structure for Robust Adversarial Alignment}

To probe internal behaviors of aligned language models under adversarial attack, we apply our Adversarial Vulnerability Quality Index (AVQI) and perform cluster-level analysis across hidden layers. This reveals the following consistent structure:

\begin{enumerate}
    \item \textbf{Safe completions form compact, low-variance clusters} in latent space, suggesting a well-regularized internal encoding of benign behavior.

    \item \textbf{Adversarial generations tend to lie deceptively close to safe completions}, often near the boundary of the safe region. This induces a \emph{camouflage effect}, where adversarial responses become representationally similar to safe ones, eluding standard alignment signals.

    \item \textbf{Ideal structure:} Robust alignment requires \emph{orthogonal separation} between safe and unsafe/adversarial behaviors. Despite differing attack modalities, unsafe and adversarial completions should coalesce into a coherent adversarial subspace.
\end{enumerate}

These findings expose a key limitation of preference-only optimization (e.g., DPO): while it enforces surface-level output behavior, it fails to impose the internal geometric structure necessary for generalization to obfuscated or unseen attacks.

To address this, we introduce a latent-space regularization objective that explicitly encourages:
\begin{itemize}[nosep,leftmargin=1em]
    \item separation of safe from adversarial representations,
    \item and consolidation of unsafe and jailbreak generations into a unified adversarial manifold.
\end{itemize}

Embedding such geometric priors during training enables the model to internalize behavioral semantics, fostering both interpretability and robustness under adversarial perturbations.




\begin{comment}
\begin{figure*}[t]
\centering
\begin{tcolorbox}[
  enhanced,
  colback=white,
  colframe=black,
  boxrule=1pt,
  borderline={0.6pt}{2pt}{black},
  sharp corners,
  width=\textwidth,
]
\vspace{-4mm}
\[
\begin{aligned}
\min_{\theta} \quad & 
\underbrace{-\log \sigma\Big(
\log \pi_\theta(y_{\mathrm{safe}} \mid x)
- \log \pi_\theta(y_{\mathrm{adv}} \mid x)
- \alpha \left[
\log \pi_{\mathrm{ref}}(y_{\mathrm{safe}} \mid x)
- \log \pi_{\mathrm{ref}}(y_{\mathrm{adv}} \mid x)
\right]
\Big)}_{\text{(1) Relaxed Preference Loss}}
\\[6pt]
& +\; \lambda \Big[
\underbrace{
\sum_{\substack{h_s \in C_{\mathrm{safe}} \\ h_a \in C_{\mathrm{adv}}}} 
\max(0,\; M - \|h_s - h_a\|_2)
}_{\text{(2) Safe--Adversarial Separation}}
\;+\;
\underbrace{
\sum_{\substack{h_u \in C_{\mathrm{unsafe}} \\ h_j \in C_{\mathrm{jb}}}} 
\max(0,\; \|h_u - h_j\|_2 - \delta)
}_{\text{(3) Unsafe--Jailbreak Merging}}
\Big]
\end{aligned}
\]
\vspace{-4mm}
\end{tcolorbox}

\vspace{-2mm}
\caption{
\textbf{Final Objective for Geometric Preference Optimization.} The total loss balances preference alignment and geometric regularization:
\begin{itemize}[noitemsep,leftmargin=1em]
    \item \textbf{(1) Relaxed Preference Loss:} Softens the KL constraint via $\alpha$ while ensuring $y_{\mathrm{safe}}$ is preferred over $y_{\mathrm{adv}}$.
    \item \textbf{(2) Safe--Adversarial Separation:} Pushes latent representations of safe and adversarial generations apart by a margin $M$.
    \item \textbf{(3) Unsafe--Jailbreak Merging:} Encourages unsafe and jailbreak responses to form a compact adversarial cluster within distance $\delta$.
\end{itemize}
Hyperparameters $\lambda$, $\alpha$, $M$, and $\delta$ jointly govern the preference-geometric balance for improved adversarial robustness.
}
\label{fig:final_objective_geometric_dpo}
\vspace{-2mm}
\end{figure*}
\end{comment}


\subsection{Latent Geometric Regularization Loss}

Motivated by the observed geometric patterns in hidden representations, we introduce a latent-space regularization objective that promotes the desired separation between behavioral classes. Our goal is twofold: (1) to enforce representational separation between safe and adversarial completions, and (2) to consolidate unsafe and jailbreak generations into a coherent adversarial subspace.

Let $h_\theta(x, y)$ denote the hidden representation of a prompt–response pair, extracted from a designated intermediate layer. We define the following sets:
\[
C_{\mathrm{safe}},\quad C_{\mathrm{unsafe}},\quad C_{\mathrm{jb}} \subset \mathbb{R}^d
\]
representing latent vectors corresponding to safe, unsafe, and jailbreak completions, respectively.

Inspired by supervised contrastive learning~\cite{khosla2020supervised} and metric learning via triplet loss~\cite{schroff2015facenet}, we define two margin-based constraints:

\vspace{1mm}
\textbf{(1) Safe–Adversarial Separation.} To increase separation between safe and adversarial representations (including both unsafe and jailbreak), we define a contrastive loss:
\[
\mathcal{L}_{\mathrm{sep}} = \sum_{\substack{h_s \in C_{\mathrm{safe}} \\ h_a \in C_{\mathrm{adv}}}} \max(0,\; M - \|h_s - h_a\|_2)
\]
where $C_{\mathrm{adv}} = C_{\mathrm{unsafe}} \cup C_{\mathrm{jb}}$ and $M$ is a minimum separation margin.

\vspace{1mm}
\textbf{(2) Unsafe–Jailbreak Consolidation.} To encourage geometric similarity between unsafe and jailbreak clusters, we introduce a proximity constraint:
\[
\mathcal{L}_{\mathrm{merge}} = \sum_{\substack{h_u \in C_{\mathrm{unsafe}} \\ h_j \in C_{\mathrm{jb}}}} \max(0,\; \|h_u - h_j\|_2 - \delta)
\]
where $\delta$ defines the maximum allowable spread within the adversarial subspace.





\vspace{1mm}
\subsection{Final Loss: Preference-Guided Geometric Optimization}

To complete the training loss, we combine the relaxed preference optimization objective with our latent cluster regularization terms. This joint objective balances behavioral alignment at the output level with geometric consistency in the hidden representation space:
\[
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{pref}} + \lambda_{\text{sep}}\, \mathcal{L}_{\mathrm{sep}} + \lambda_{\text{merge}}\, \mathcal{L}_{\mathrm{merge}}
\]
Here, $\mathcal{L}_{\text{pref}}$ represents the primary preference optimization term, which encourages the model to assign higher likelihood to safe completions over adversarial ones. The auxiliary terms, $\mathcal{L}_{\mathrm{sep}}$ and $\mathcal{L}_{\mathrm{merge}}$, impose geometric constraints on the model's latent space. Specifically, $\mathcal{L}_{\mathrm{sep}}$ increases the representational distance between safe and adversarial examples, while $\mathcal{L}_{\mathrm{merge}}$ encourages unsafe and jailbreak generations to occupy a shared adversarial subspace. The corresponding weights $\lambda_{\text{sep}}$ and $\lambda_{\text{merge}}$ balance the influence of these geometric regularizers relative to the main alignment objective.

This composite loss guides the model to:
\begin{itemize}[nosep,leftmargin=1.5em]
    \item Align with preference annotations by preferring safe responses over adversarial ones ($\mathcal{L}_{\text{pref}}$),
    \item Create latent separation between safe and adversarial behaviors ($\mathcal{L}_{\mathrm{sep}}$),
    \item Geometrically unify unsafe and jailbreak completions into a compact adversarial cluster ($\mathcal{L}_{\mathrm{merge}}$).
\end{itemize}

This objective integrates output-level supervision with latent-space structuring, fostering alignment in the model’s predictions and the internal representation space, enabling more generalizable and mechanistically grounded adversarial robustness.










\subsection{Expanded Final Loss with Learned Pooled Representations}

The structure of the total alignment loss remains unchanged:
\[
\mathcal{L}_{\mathrm{total}} = \mathcal{L}_{\mathrm{pref}} + \lambda_{\mathrm{sep}} \cdot \mathcal{L}_{\mathrm{sep}} + \lambda_{\mathrm{merge}} \cdot \mathcal{L}_{\mathrm{merge}}
\]
However, the internal computation of $\mathcal{L}_{\mathrm{sep}}$ and $\mathcal{L}_{\mathrm{merge}}$ is transformed by the learned attention profile $\alpha^{(l)}$.

\vspace{1mm}
\noindent\textbf{Old setting (before attention pooling):} Representations were extracted only from the final layer:
\[
\tilde{h}_y = h_y^{(L)}
\]

\vspace{1mm}
\noindent\textbf{New setting (after attention pooling):} Representations are computed as a weighted sum across layers:
\[
\tilde{h}_y = \sum_{l=1}^{L} \alpha^{(l)} h_y^{(l)}, \quad \text{where } \sum_l \alpha^{(l)} = 1,\; \alpha^{(l)} \geq 0
\]

This change impacts both latent terms in the loss.

\vspace{1mm}
\noindent\textbf{Expanded $\mathcal{L}_{\mathrm{sep}}$:}
\[
\begin{aligned}
\mathcal{L}_{\mathrm{sep}} &=
\max\left(0,\; M - \left\| \sum_{l=1}^L \alpha^{(l)} \left( h^{(l)}_{\text{safe}} - h^{(l)}_{\text{unsafe}} \right) \right\|_2 \right) \\
&\quad + \max\left(0,\; M - \left\| \sum_{l=1}^L \alpha^{(l)} \left( h^{(l)}_{\text{safe}} - h^{(l)}_{\text{jb}} \right) \right\|_2 \right)
\end{aligned}
\]

\vspace{1mm}
\noindent\textbf{Expanded $\mathcal{L}_{\mathrm{merge}}$:}
\[
\mathcal{L}_{\mathrm{merge}} =
\max\left(0,\; \left\| \sum_{l=1}^L \alpha^{(l)} \left( h^{(l)}_{\text{unsafe}} - h^{(l)}_{\text{jb}} \right) \right\|_2 - \delta \right)
\]

This formulation shows how $\alpha^{(l)}$ actively controls the distance computation across layers — creating a soft projection of geometric behavior that blends semantic signals from multiple layers.

\vspace{1mm}
\noindent\textbf{Gradient Flow.}
If $\alpha$ is treated as trainable, gradients from $\mathcal{L}_{\mathrm{sep}}$ and $\mathcal{L}_{\mathrm{merge}}$ flow through the weighted differences:
\[
\nabla_{\alpha^{(l)}} \mathcal{L}_{\mathrm{merge}},\quad \nabla_{\alpha^{(l)}} \mathcal{L}_{\mathrm{sep}} \neq 0
\]

\noindent If $\alpha$ is fixed (pre-trained), these terms are treated as constants during optimization of model parameters.

\vspace{1mm}
\noindent\textbf{Impact.} \\
By replacing static single-layer representations with weighted layerwise combinations, this updated loss:
\begin{itemize}[leftmargin=1.5em]
    \item Induces richer geometry across behavior types (safe, unsafe, jailbreak).
    \item Avoids overfitting to a specific depth (e.g., last layer).
    \item Enables generalization via attention-tuned latent spaces.
\end{itemize}

\subsection{Relaxing KL Constraints: From DPO to GRPO}

Direct Preference Optimization (DPO)~\cite{rafailov2023direct} optimizes a pairwise logistic preference loss, with a KL-like term that constrains divergence from a reference model:
\[
\mathcal{L}_{\mathrm{DPO}} = -\log \sigma\left(
\log \pi_\theta(y_{\mathrm{safe}} \mid x) -
\log \pi_\theta(y_{\mathrm{unsafe}} \mid x) -
\Delta_{\mathrm{ref}}
\right)
\]
where
\[
\Delta_{\mathrm{ref}} =
\log \pi_{\mathrm{ref}}(y_{\mathrm{safe}} \mid x) -
\log \pi_{\mathrm{ref}}(y_{\mathrm{unsafe}} \mid x)
\]

This reference term acts as a surrogate for the reverse KL between the learned policy $\pi_\theta$ and the reference policy $\pi_{\mathrm{ref}}$, and helps stabilize training by preventing undesirable mode collapse. However, it also limits flexibility—especially when the reference model itself may be poorly calibrated or unsafe under adversarial conditions.

\vspace{1mm}
\textbf{From KL Constraints to Controlled Drift.} \\
Inspired by recent advances such as GRPO~\cite{wu2024generalized} and $\varepsilon$-DPO~\cite{chen2023epsilon}, we propose a relaxed version of the preference loss that introduces an adjustable scale $\alpha \in [0,1]$:
\[
\mathcal{L}_{\mathrm{pref}} = -\log \sigma\left(
\log \pi_\theta(y_{\mathrm{safe}} \mid x) -
\log \pi_\theta(y_{\mathrm{adv}} \mid x) -
\alpha \Delta_{\mathrm{ref}}
\right)
\]

Here, $\alpha$ governs the strength of the KL regularization. When $\alpha = 1$, we recover standard DPO. When $\alpha = 0$, the loss becomes fully reference-free, letting the model optimize preferences without constraint. This relaxation allows the policy to learn safer completions even when the reference model fails to differentiate between benign and adversarial outputs.

\vspace{1mm}
\textbf{Toward Structured Alignment.} \\
While $\mathcal{L}_{\mathrm{pref}}$ guides behavioral preference at the output level, it lacks any structural incentive for how safe and adversarial examples should be represented internally. To address this, we incorporate latent-space supervision via our learned pooled representations $\tilde{h}_y = \sum_l \alpha^{(l)} h_y^{(l)}$.

The full training objective becomes:
\[
\mathcal{L}_{\mathrm{total}} =
\mathcal{L}_{\mathrm{pref}} +
\lambda_{\mathrm{sep}} \cdot \mathcal{L}_{\mathrm{sep}} +
\lambda_{\mathrm{merge}} \cdot \mathcal{L}_{\mathrm{merge}}
\]

Here:
\begin{itemize}[leftmargin=1.5em]
    \item $\mathcal{L}_{\mathrm{pref}}$ is the relaxed DPO loss above,
    \item $\mathcal{L}_{\mathrm{sep}}$ encourages geometric separation of safe vs. adversarial completions, and
    \item $\mathcal{L}_{\mathrm{merge}}$ ensures unsafe and jailbreak examples reside in a unified adversarial subspace.
\end{itemize}

This formulation allows preference alignment and latent geometry to be learned in tandem, while avoiding over-reliance on an imperfect reference policy.



\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/results.png}
    \caption{
    \textbf{Adversarial Robustness Across LLMs: Baseline vs. DPO vs. GRACE}
    This heatmap illustrates Attack Success Rates (ASR, in \%) across various adversarial attacks for 21 popular LLMs under three training configurations: baseline (original model), DPO fine-tuning, and our proposed GRACE fine-tuning. Rows correspond to adversarial attacks grouped into three broad categories: \emph{Jailbreak}, \emph{Control Hijacking}, and \emph{Degradation}. Columns are grouped by model, each with three versions: Baseline, DPO, and GRACE. 
    \textbf{Key observations:} (1) DPO offers modest ASR reduction (2–5\% on average); (2) GRACE significantly reduces ASR (35–39\% reduction); (3) Models like GPT-4 and Mixtral show substantial improvements across high-risk attacks (e.g., DAN, Goal Hijack, and BadChain). The intense color contrast shows that GRACE consistently outperforms DPO in neutralizing adversarial completions while preserving generalization across model scales and families.
    }
    \label{fig:asr_heatmap_grace}
\end{figure*}





\begin{figure*}[t]
\centering
\begin{tcolorbox}[
  enhanced,
  colback=white,
  colframe=black,
  boxrule=1pt,
  borderline={0.6pt}{2pt}{black},
  sharp corners,
  width=\textwidth,
]
\vspace{-4mm}
\[
\begin{aligned}
\min_{\theta} \quad & 
\underbrace{-\log \sigma\left(
\log \pi_\theta(y_{\mathrm{safe}} \mid x)
- \log \pi_\theta(y_{\mathrm{adv}} \mid x)
- \alpha \big[
\log \pi_{\mathrm{ref}}(y_{\mathrm{safe}} \mid x)
- \log \pi_{\mathrm{ref}}(y_{\mathrm{adv}} \mid x)
\big]
\right)}_{\text{(1) Relaxed Preference Loss}} \\[6pt]
& +\; \lambda_{\mathrm{sep}} \cdot
\underbrace{
\left[
\max\left(0,\; M - \left\| \tilde{h}_{\mathrm{safe}} - \tilde{h}_{\mathrm{unsafe}} \right\|_2 \right)
+
\max\left(0,\; M - \left\| \tilde{h}_{\mathrm{safe}} - \tilde{h}_{\mathrm{jb}} \right\|_2 \right)
\right]
}_{\text{(2) Safe--Adversarial Latent Separation}} \\[6pt]
& +\; \lambda_{\mathrm{merge}} \cdot
\underbrace{
\max\left(0,\; \left\| \tilde{h}_{\mathrm{unsafe}} - \tilde{h}_{\mathrm{jb}} \right\|_2 - \delta \right)
}_{\text{(3) Unsafe--Jailbreak Latent Merging}}
\end{aligned}
\]
\vspace{-4mm}
\end{tcolorbox}

\vspace{-2mm}
\caption{
\textbf{Final Objective for Geometric Preference Optimization.} This loss integrates relaxed preference alignment with latent-space regularization using pooled representations $\tilde{h}_y = \sum_l \alpha^{(l)} h_y^{(l)}$:
\begin{itemize}[noitemsep,leftmargin=1em]
    \item \textbf{(1) Relaxed Preference Loss:} Generalizes DPO by introducing a scaling factor $\alpha$ over the reference model KL constraint $\Delta_{\mathrm{ref}}$, improving robustness when $\pi_{\mathrm{ref}}$ is unsafe.
    \item \textbf{(2) Latent Separation:} Encourages margin-based distancing between safe and both unsafe/jailbreak representations using $\tilde{h}_y$.
    \item \textbf{(3) Latent Merging:} Promotes representational cohesion between unsafe and jailbreak examples within a threshold $\delta$.
\end{itemize}
All latent terms operate on frozen LLM representations pooled via $\alpha^{(l)}$, while gradients flow only into the policy $\pi_\theta$ and optionally $\alpha$. Hyperparameters $(\alpha, \lambda_{\mathrm{sep}}, \lambda_{\mathrm{merge}}, M, \delta)$ control the trade-off between behavioral fidelity and latent alignment.
}
\label{fig:final_objective_geometric_dpo}
\vspace{-2mm}
\end{figure*}

==> fusion_examples/all_comedy.tex <==
==========Qwen3=============


\textcolor[HTML]{2B4239}{Yes, }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{comedian's }\textcolor[HTML]{2B4239}{use }\textcolor[HTML]{2B4239}{of }\textcolor[HTML]{2B4239}{\textbf{audience }\textcolor[HTML]{2B4239}{interaction} }\textcolor[HTML]{2B4239}{can }\textcolor[HTML]{2B4239}{significantly }\textcolor[HTML]{2B4239}{enhance }\textcolor[HTML]{2B4239}{both }\textcolor[HTML]{2B4239}{their }\textcolor[HTML]{2B4239}{\textbf{delivery} }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{2B4239}{\textbf{stage }\textcolor[HTML]{2B4239}{presence}. }\textcolor[HTML]{2B4239}{When }\textcolor[HTML]{2B4239}{used }\textcolor[HTML]{2B4239}{effectively, }\textcolor[HTML]{2B4239}{audience }\textcolor[HTML]{2B4239}{interaction }\textcolor[HTML]{2B4239}{can }\textcolor[HTML]{2B4239}{transform }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{standard }\textcolor[HTML]{2B4239}{stand-up }\textcolor[HTML]{2B4239}{performance }\textcolor[HTML]{2B4239}{into }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{more }\textcolor[HTML]{2B4239}{dynamic, }\textcolor[HTML]{2B4239}{engaging, }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{2B4239}{memorable }\textcolor[HTML]{2B4239}{experience. }\textcolor[HTML]{2B4239}{Here's }\textcolor[HTML]{2B4239}{how:\\}\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{2B4239}{---\\}\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{2B4239}{\#\#\# }\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{\textbf{Enhances }\textcolor[HTML]{2B4239}{Delivery}\\}\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{2B4239}{1. }\textcolor[HTML]{2B4239}{\textbf{Creates }\textcolor[HTML]{2B4239}{Natural }\textcolor[HTML]{2B4239}{Rhythm }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{2B4239}{Pacing}\\}\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{Interacting }\textcolor[HTML]{2B4239}{with }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{audience }\textcolor[HTML]{2B4239}{can }\textcolor[HTML]{2B4239}{break }\textcolor[HTML]{2B4239}{up }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{monotony }\textcolor[HTML]{2B4239}{of }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{scripted }\textcolor[HTML]{2B4239}{set, }\textcolor[HTML]{2B4239}{allowing }\textcolor[HTML]{2B4239}{for }\textcolor[HTML]{2B4239}{natural }\textcolor[HTML]{2B4239}{pauses, }\textcolor[HTML]{2B4239}{laughs, }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{2B4239}{transitions. }\textcolor[HTML]{2B4239}{This }\textcolor[HTML]{2B4239}{variation }\textcolor[HTML]{2B4239}{in }\textcolor[HTML]{2B4239}{pacing }\textcolor[HTML]{2B4239}{can }\textcolor[HTML]{2B4239}{make }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{performance }\textcolor[HTML]{2B4239}{feel }\textcolor[HTML]{2B4239}{more }\textcolor[HTML]{2B4239}{spontaneous }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{2B4239}{alive.\\}\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{2B4239}{2. }\textcolor[HTML]{2B4239}{\textbf{Provides }\textcolor[HTML]{2B4239}{Real-Time }\textcolor[HTML]{2B4239}{Feedback}\\}\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{ }\textcolor[HTML]{2B4239}{Audience }\textcolor[HTML]{2B4239}{reactions }\textcolor[HTML]{2B4239}{during }\textcolor[HTML]{2B4239}{interactions }\textcolor[HTML]{2B4239}{give }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{comedian }\textcolor[HTML]{2B4239}{immediate }\textcolor[HTML]{2B4239}{feedback, }\textcolor[HTML]{2B4239}{helping}...


==========Gemma3=============


\textcolor[HTML]{CA492D}{Absolutely! }\textcolor[HTML]{CA492D}{A }\textcolor[HTML]{CA492D}{comedian's }\textcolor[HTML]{CA492D}{use }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{CA492D}{interaction }\textcolor[HTML]{CA492D}{can }\textcolor[HTML]{CA492D}{\textit{significantly} }\textcolor[HTML]{CA492D}{enhance }\textcolor[HTML]{CA492D}{their }\textcolor[HTML]{CA492D}{delivery }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{stage }\textcolor[HTML]{CA492D}{presence. }\textcolor[HTML]{CA492D}{It's }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{powerful }\textcolor[HTML]{CA492D}{tool, }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{when }\textcolor[HTML]{CA492D}{done }\textcolor[HTML]{CA492D}{well, }\textcolor[HTML]{CA492D}{it's }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{huge }\textcolor[HTML]{CA492D}{part }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{CA492D}{what }\textcolor[HTML]{CA492D}{separates }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{good }\textcolor[HTML]{CA492D}{comedian }\textcolor[HTML]{CA492D}{from }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{\textit{great} }\textcolor[HTML]{CA492D}{one. }\textcolor[HTML]{CA492D}{Here's }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{breakdown }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{CA492D}{how }\textcolor[HTML]{CA492D}{it }\textcolor[HTML]{CA492D}{works, }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{benefits:\\}\textcolor[HTML]{CA492D}{\\}\textcolor[HTML]{CA492D}{\textbf{How }\textcolor[HTML]{CA492D}{Audience }\textcolor[HTML]{CA492D}{Interaction }\textcolor[HTML]{CA492D}{Enhances }\textcolor[HTML]{CA492D}{Delivery }\textcolor[HTML]{CA492D}{\& }\textcolor[HTML]{CA492D}{Stage }\textcolor[HTML]{CA492D}{Presence:}\\}\textcolor[HTML]{CA492D}{\\}\textcolor[HTML]{CA492D}{* }\textcolor[HTML]{CA492D}{\textbf{Breaks }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{Fourth }\textcolor[HTML]{CA492D}{Wall:} }\textcolor[HTML]{CA492D}{It }\textcolor[HTML]{CA492D}{immediately }\textcolor[HTML]{CA492D}{makes }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{performance }\textcolor[HTML]{CA492D}{less }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{one-way }\textcolor[HTML]{CA492D}{lecture }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{more }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{shared }\textcolor[HTML]{CA492D}{experience. }\textcolor[HTML]{CA492D}{This }\textcolor[HTML]{CA492D}{creates }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{more }\textcolor[HTML]{CA492D}{intimate }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{engaging }\textcolor[HTML]{CA492D}{atmosphere.\\}\textcolor[HTML]{CA492D}{\textit{ }\textcolor[HTML]{CA492D}{\textbf{Improves }\textcolor[HTML]{CA492D}{Timing }\textcolor[HTML]{CA492D}{\& }\textcolor[HTML]{CA492D}{Reactivity:} }\textcolor[HTML]{CA492D}{ }\textcolor[HTML]{CA492D}{Good }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{CA492D}{work }\textcolor[HTML]{CA492D}{forces }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{comedian }\textcolor[HTML]{CA492D}{to }\textcolor[HTML]{CA492D}{be }\textcolor[HTML]{CA492D}{}present* }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{react }\textcolor[HTML]{CA492D}{in }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{moment. }\textcolor[HTML]{CA492D}{ }\textcolor[HTML]{CA492D}{This }\textcolor[HTML]{CA492D}{sharpens }\textcolor[HTML]{CA492D}{their }\textcolor[HTML]{CA492D}{comedic }\textcolor[HTML]{CA492D}{timing, }\textcolor[HTML]{CA492D}{as }\textcolor[HTML]{CA492D}{they }\textcolor[HTML]{CA492D}{have }\textcolor[HTML]{CA492D}{to}...


==========DeepSeek-V3=============


\textcolor[HTML]{9B60AA}{Absolutely! }\textcolor[HTML]{9B60AA}{A }\textcolor[HTML]{9B60AA}{comedian's }\textcolor[HTML]{9B60AA}{use }\textcolor[HTML]{9B60AA}{of }\textcolor[HTML]{9B60AA}{audience }\textcolor[HTML]{9B60AA}{interaction }\textcolor[HTML]{9B60AA}{can }\textcolor[HTML]{9B60AA}{significantly }\textcolor[HTML]{9B60AA}{enhance }\textcolor[HTML]{9B60AA}{their }\textcolor[HTML]{9B60AA}{delivery }\textcolor[HTML]{9B60AA}{and }\textcolor[HTML]{9B60AA}{stage }\textcolor[HTML]{9B60AA}{presence }\textcolor[HTML]{9B60AA}{in }\textcolor[HTML]{9B60AA}{several }\textcolor[HTML]{9B60AA}{ways:\\}\textcolor[HTML]{9B60AA}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{9B60AA}{1. }\textcolor[HTML]{9B60AA}{\textbf{Engagement }\textcolor[HTML]{9B60AA}{\& }\textcolor[HTML]{9B60AA}{Connection}\\}\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{9B60AA}{Direct }\textcolor[HTML]{9B60AA}{interaction }\textcolor[HTML]{9B60AA}{makes }\textcolor[HTML]{9B60AA}{the }\textcolor[HTML]{9B60AA}{audience }\textcolor[HTML]{9B60AA}{feel }\textcolor[HTML]{9B60AA}{involved, }\textcolor[HTML]{9B60AA}{creating }\textcolor[HTML]{9B60AA}{a }\textcolor[HTML]{9B60AA}{personal }\textcolor[HTML]{9B60AA}{connection }\textcolor[HTML]{9B60AA}{that }\textcolor[HTML]{9B60AA}{boosts }\textcolor[HTML]{9B60AA}{engagement.\\}\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{9B60AA}{It }\textcolor[HTML]{9B60AA}{breaks }\textcolor[HTML]{9B60AA}{the }\textcolor[HTML]{9B60AA}{"fourth }\textcolor[HTML]{9B60AA}{wall," }\textcolor[HTML]{9B60AA}{making }\textcolor[HTML]{9B60AA}{the }\textcolor[HTML]{9B60AA}{performance }\textcolor[HTML]{9B60AA}{feel }\textcolor[HTML]{9B60AA}{more }\textcolor[HTML]{9B60AA}{spontaneous }\textcolor[HTML]{9B60AA}{and }\textcolor[HTML]{9B60AA}{alive.\\}\textcolor[HTML]{9B60AA}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{9B60AA}{2. }\textcolor[HTML]{9B60AA}{\textbf{Adaptability }\textcolor[HTML]{9B60AA}{\& }\textcolor[HTML]{9B60AA}{Improvisation}\\}\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{9B60AA}{Skilled }\textcolor[HTML]{9B60AA}{crowd }\textcolor[HTML]{9B60AA}{work }\textcolor[HTML]{9B60AA}{demonstrates }\textcolor[HTML]{9B60AA}{quick }\textcolor[HTML]{9B60AA}{wit, }\textcolor[HTML]{9B60AA}{making }\textcolor[HTML]{9B60AA}{the }\textcolor[HTML]{9B60AA}{material }\textcolor[HTML]{9B60AA}{feel }\textcolor[HTML]{9B60AA}{fresh }\textcolor[HTML]{9B60AA}{and }\textcolor[HTML]{9B60AA}{unique }\textcolor[HTML]{9B60AA}{to }\textcolor[HTML]{9B60AA}{each }\textcolor[HTML]{9B60AA}{show.\\}\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{9B60AA}{It }\textcolor[HTML]{9B60AA}{allows }\textcolor[HTML]{9B60AA}{comedians }\textcolor[HTML]{9B60AA}{to }\textcolor[HTML]{9B60AA}{riff }\textcolor[HTML]{9B60AA}{off }\textcolor[HTML]{9B60AA}{real-time }\textcolor[HTML]{9B60AA}{reactions, }\textcolor[HTML]{9B60AA}{adding }\textcolor[HTML]{9B60AA}{unpredictability }\textcolor[HTML]{9B60AA}{and }\textcolor[HTML]{9B60AA}{excitement.\\}\textcolor[HTML]{9B60AA}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{9B60AA}{3. }\textcolor[HTML]{9B60AA}{\textbf{Energy }\textcolor[HTML]{9B60AA}{\& }\textcolor[HTML]{9B60AA}{Authenticity}\\}\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{ }\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{9B60AA}{A }\textcolor[HTML]{9B60AA}{dynamic }\textcolor[HTML]{9B60AA}{back-and-forth }\textcolor[HTML]{9B60AA}{keeps }\textcolor[HTML]{9B60AA}{the }\textcolor[HTML]{9B60AA}{energy }\textcolor[HTML]{9B60AA}{high}...


==========CommandA=============


\textcolor[HTML]{2D4CB9}{Absolutely, }\textcolor[HTML]{2D4CB9}{a }\textcolor[HTML]{2D4CB9}{comedian's }\textcolor[HTML]{2D4CB9}{use }\textcolor[HTML]{2D4CB9}{of }\textcolor[HTML]{2D4CB9}{audience }\textcolor[HTML]{2D4CB9}{interaction }\textcolor[HTML]{2D4CB9}{can }\textcolor[HTML]{2D4CB9}{significantly }\textcolor[HTML]{2D4CB9}{enhance }\textcolor[HTML]{2D4CB9}{their }\textcolor[HTML]{2D4CB9}{delivery }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{stage }\textcolor[HTML]{2D4CB9}{presence }\textcolor[HTML]{2D4CB9}{in }\textcolor[HTML]{2D4CB9}{several }\textcolor[HTML]{2D4CB9}{ways:\\}\textcolor[HTML]{2D4CB9}{\\}\textcolor[HTML]{2D4CB9}{1. }\textcolor[HTML]{2D4CB9}{\textbf{Engagement }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{Connection}: }\textcolor[HTML]{2D4CB9}{Interacting }\textcolor[HTML]{2D4CB9}{with }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{audience }\textcolor[HTML]{2D4CB9}{creates }\textcolor[HTML]{2D4CB9}{a }\textcolor[HTML]{2D4CB9}{sense }\textcolor[HTML]{2D4CB9}{of }\textcolor[HTML]{2D4CB9}{inclusion }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{connection. }\textcolor[HTML]{2D4CB9}{When }\textcolor[HTML]{2D4CB9}{a }\textcolor[HTML]{2D4CB9}{comedian }\textcolor[HTML]{2D4CB9}{involves }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{audience }\textcolor[HTML]{2D4CB9}{directly, }\textcolor[HTML]{2D4CB9}{it }\textcolor[HTML]{2D4CB9}{breaks }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{fourth }\textcolor[HTML]{2D4CB9}{wall }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{makes }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{performance }\textcolor[HTML]{2D4CB9}{feel }\textcolor[HTML]{2D4CB9}{more }\textcolor[HTML]{2D4CB9}{personal }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{intimate. }\textcolor[HTML]{2D4CB9}{This }\textcolor[HTML]{2D4CB9}{engagement }\textcolor[HTML]{2D4CB9}{can }\textcolor[HTML]{2D4CB9}{lead }\textcolor[HTML]{2D4CB9}{to }\textcolor[HTML]{2D4CB9}{a }\textcolor[HTML]{2D4CB9}{more }\textcolor[HTML]{2D4CB9}{receptive }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{responsive }\textcolor[HTML]{2D4CB9}{crowd, }\textcolor[HTML]{2D4CB9}{which }\textcolor[HTML]{2D4CB9}{in }\textcolor[HTML]{2D4CB9}{turn }\textcolor[HTML]{2D4CB9}{boosts }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{comedian's }\textcolor[HTML]{2D4CB9}{confidence }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{energy }\textcolor[HTML]{2D4CB9}{on }\textcolor[HTML]{2D4CB9}{stage.\\}\textcolor[HTML]{2D4CB9}{\\}\textcolor[HTML]{2D4CB9}{ }\textcolor[HTML]{2D4CB9}{\textbf{Example}: }\textcolor[HTML]{2D4CB9}{Asking }\textcolor[HTML]{2D4CB9}{for }\textcolor[HTML]{2D4CB9}{volunteers }\textcolor[HTML]{2D4CB9}{or }\textcolor[HTML]{2D4CB9}{incorporating }\textcolor[HTML]{2D4CB9}{audience }\textcolor[HTML]{2D4CB9}{members }\textcolor[HTML]{2D4CB9}{into }\textcolor[HTML]{2D4CB9}{bits }\textcolor[HTML]{2D4CB9}{can }\textcolor[HTML]{2D4CB9}{create }\textcolor[HTML]{2D4CB9}{memorable }\textcolor[HTML]{2D4CB9}{moments }\textcolor[HTML]{2D4CB9}{that }\textcolor[HTML]{2D4CB9}{resonate }\textcolor[HTML]{2D4CB9}{with }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{entire }\textcolor[HTML]{2D4CB9}{crowd.\\}\textcolor[HTML]{2D4CB9}{\\}\textcolor[HTML]{2D4CB9}{2. }\textcolor[HTML]{2D4CB9}{\textbf{Improvisation }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{Adaptability}: }\textcolor[HTML]{2D4CB9}{Au}...

==> fusion_examples/comedy_long.tex <==
\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{2B4239}{Yes, }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{comedian's }\textcolor[HTML]{2B4239}{use }\textcolor[HTML]{2B4239}{of }\textcolor[HTML]{2B4239}{\textbf{audience }\textcolor[HTML]{2B4239}{interaction} }\textcolor[HTML]{2B4239}{can }\textcolor[HTML]{2B4239}{significantly }\textcolor[HTML]{2B4239}{enhance }\textcolor[HTML]{2B4239}{both }\textcolor[HTML]{2B4239}{their }\textcolor[HTML]{2B4239}{\textbf{delivery} }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{2B4239}{\textbf{stage }\textcolor[HTML]{2B4239}{presence}. }\textcolor[HTML]{2B4239}{When }\textcolor[HTML]{2B4239}{executed }\textcolor[HTML]{2D4CB9}{skillfully, }\textcolor[HTML]{2D4CB9}{it }\textcolor[HTML]{CA492D}{transforms }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{standard }\textcolor[HTML]{2B4239}{stand-up }\textcolor[HTML]{2B4239}{performance }\textcolor[HTML]{2B4239}{into }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{dynamic, }\textcolor[HTML]{2B4239}{engaging, }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{CA492D}{personalized }\textcolor[HTML]{2B4239}{experience. }\textcolor[HTML]{2B4239}{Here’s }\textcolor[HTML]{2B4239}{how:\\}\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{CA492D}{\textbf{Enhancing }\textcolor[HTML]{2B4239}{Delivery}\\}\textcolor[HTML]{2D4CB9}{1. }\textcolor[HTML]{CA492D}{\textbf{Improves }\textcolor[HTML]{CA492D}{Timing }\textcolor[HTML]{CA492D}{\& }\textcolor[HTML]{2D4CB9}{Reactivity}: }\textcolor[HTML]{2D4CB9}{Audience }\textcolor[HTML]{2D4CB9}{interaction }\textcolor[HTML]{CA492D}{forces }\textcolor[HTML]{BBB1A4}{comedians }\textcolor[HTML]{CA492D}{to }\textcolor[HTML]{CA492D}{be }\textcolor[HTML]{2D4CB9}{present }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{2D4CB9}{adapt }\textcolor[HTML]{CA492D}{in }\textcolor[HTML]{BBB1A4}{real-time, }\textcolor[HTML]{BBB1A4}{sharpening }\textcolor[HTML]{CA492D}{their }\textcolor[HTML]{CA492D}{comedic }\textcolor[HTML]{CA492D}{timing }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{8E8572}{improvisation }\textcolor[HTML]{8E8572}{skills.\\}\textcolor[HTML]{2B4239}{2. }\textcolor[HTML]{2B4239}{\textbf{Creates }\textcolor[HTML]{2B4239}{Natural }\textcolor[HTML]{BBB1A4}{Rhythm}: }\textcolor[HTML]{9B60AA}{It }\textcolor[HTML]{9B60AA}{breaks }\textcolor[HTML]{2B4239}{up }\textcolor[HTML]{2B4239}{scripted }\textcolor[HTML]{2B4239}{material, }\textcolor[HTML]{2B4239}{adding }\textcolor[HTML]{BBB1A4}{spontaneity }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{9B60AA}{keeping }\textcolor[HTML]{9B60AA}{the }\textcolor[HTML]{9B60AA}{performance }\textcolor[HTML]{9B60AA}{lively.\\}\textcolor[HTML]{2B4239}{3. }\textcolor[HTML]{2B4239}{\textbf{Allows }\textcolor[HTML]{2B4239}{for }\textcolor[HTML]{2B4239}{Callbacks }\textcolor[HTML]{9B60AA}{\& }\textcolor[HTML]{BBB1A4}{Customization}: }\textcolor[HTML]{CA492D}{Referencing }\textcolor[HTML]{2B4239}{earlier }\textcolor[HTML]{2B4239}{interactions }\textcolor[HTML]{2B4239}{or }\textcolor[HTML]{2B4239}{tailoring }\textcolor[HTML]{2B4239}{jokes }\textcolor[HTML]{2B4239}{to }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{crowd’s }\textcolor[HTML]{2B4239}{responses }\textcolor[HTML]{2B4239}{makes }\textcolor[HTML]{8E8572}{the }\textcolor[HTML]{8E8572}{material }\textcolor[HTML]{8E8572}{feel }\textcolor[HTML]{8E8572}{fresh }\textcolor[HTML]{9B60AA}{and }\textcolor[HTML]{2B4239}{relevant.\\}\textcolor[HTML]{2B4239}{\\}\textcolor[HTML]{2B4239}{\#\#\# }\textcolor[HTML]{CA492D}{\textbf{Boosting }\textcolor[HTML]{2B4239}{Stage }\textcolor[HTML]{2B4239}{Presence}\\}\textcolor[HTML]{2B4239}{1. }\textcolor[HTML]{2B4239}{\textbf{Builds }\textcolor[HTML]{2B4239}{Connection }\textcolor[HTML]{BBB1A4}{\& }\textcolor[HTML]{BBB1A4}{Trust}: }\textcolor[HTML]{BBB1A4}{Breaking }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{"fourth }\textcolor[HTML]{2B4239}{wall" }\textcolor[HTML]{2B4239}{fosters }\textcolor[HTML]{2B4239}{intimacy }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{makes }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{CA492D}{feel }\textcolor[HTML]{CA492D}{valued, }\textcolor[HTML]{BBB1A4}{strengthening }\textcolor[HTML]{8E8572}{the }\textcolor[HTML]{CA492D}{comedian’s }\textcolor[HTML]{2B4239}{presence.\\}\textcolor[HTML]{2B4239}{2. }\textcolor[HTML]{CA492D}{\textbf{Showcases }\textcolor[HTML]{CA492D}{Confidence }\textcolor[HTML]{CA492D}{\& }\textcolor[HTML]{BBB1A4}{Control}: }\textcolor[HTML]{9B60AA}{Handling }\textcolor[HTML]{9B60AA}{unpredictable }\textcolor[HTML]{2B4239}{responses }\textcolor[HTML]{2B4239}{with }\textcolor[HTML]{2B4239}{humor }\textcolor[HTML]{8E8572}{demonstrates }\textcolor[HTML]{BBB1A4}{quick }\textcolor[HTML]{2D4CB9}{thinking }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{8E8572}{professionalism.\\}\textcolor[HTML]{2B4239}{3. }\textcolor[HTML]{2B4239}{\textbf{Humanizes }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{BBB1A4}{Performer}: }\textcolor[HTML]{2B4239}{Sharing }\textcolor[HTML]{9B60AA}{moments }\textcolor[HTML]{2D4CB9}{with }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{2D4CB9}{audience }\textcolor[HTML]{2B4239}{makes }\textcolor[HTML]{2B4239}{the }\textcolor[HTML]{2B4239}{comedian }\textcolor[HTML]{2B4239}{more }\textcolor[HTML]{2B4239}{relatable }\textcolor[HTML]{2B4239}{and }\textcolor[HTML]{9B60AA}{approachable.\\}\textcolor[HTML]{9B60AA}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{CA492D}{\textbf{Types }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{CA492D}{Audience }\textcolor[HTML]{9B60AA}{Interaction}\\}\textcolor[HTML]{2B4239}{- }\textcolor[HTML]{CA492D}{\textbf{Call }\textcolor[HTML]{CA492D}{\& }\textcolor[HTML]{2B4239}{Response}: }\textcolor[HTML]{BBB1A4}{Builds }\textcolor[HTML]{CA492D}{energy }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{involvement.\\}\textcolor[HTML]{BBB1A4}{- }\textcolor[HTML]{CA492D}{\textbf{Heckle }\textcolor[HTML]{BBB1A4}{Responses}: }\textcolor[HTML]{CA492D}{Risky }\textcolor[HTML]{CA492D}{but }\textcolor[HTML]{9B60AA}{rewarding }\textcolor[HTML]{BBB1A4}{when }\textcolor[HTML]{CA492D}{handled }\textcolor[HTML]{BBB1A4}{with }\textcolor[HTML]{CA492D}{wit.\\}\textcolor[HTML]{BBB1A4}{- }\textcolor[HTML]{CA492D}{\textbf{Playful }\textcolor[HTML]{BBB1A4}{Banter}: }\textcolor[HTML]{BBB1A4}{Engages }\textcolor[HTML]{CA492D}{specific }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{CA492D}{members }\textcolor[HTML]{CA492D}{while }\textcolor[HTML]{BBB1A4}{maintaining }\textcolor[HTML]{CA492D}{sensitivity.\\}\textcolor[HTML]{BBB1A4}{- }\textcolor[HTML]{CA492D}{\textbf{Improvised }\textcolor[HTML]{BBB1A4}{Bits}: }\textcolor[HTML]{CA492D}{High-level }\textcolor[HTML]{BBB1A4}{crowd }\textcolor[HTML]{CA492D}{work }\textcolor[HTML]{BBB1A4}{that }\textcolor[HTML]{CA492D}{showcases }\textcolor[HTML]{CA492D}{exceptional }\textcolor[HTML]{9B60AA}{skills.\\}\textcolor[HTML]{9B60AA}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{9B60AA}{\textbf{Potential }\textcolor[HTML]{8E8572}{Pitfalls}\\}\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{BBB1A4}{\textbf{Bombing}: }\textcolor[HTML]{BBB1A4}{Interactions }\textcolor[HTML]{9B60AA}{can }\textcolor[HTML]{CA492D}{fall }\textcolor[HTML]{CA492D}{flat, }\textcolor[HTML]{BBB1A4}{killing }\textcolor[HTML]{CA492D}{momentum.\\}\textcolor[HTML]{BBB1A4}{- }\textcolor[HTML]{CA492D}{\textbf{Offending }\textcolor[HTML]{BBB1A4}{Someone}: }\textcolor[HTML]{2D4CB9}{Missteps }\textcolor[HTML]{CA492D}{can }\textcolor[HTML]{8E8572}{alienate }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{CA492D}{members.\\}\textcolor[HTML]{BBB1A4}{- }\textcolor[HTML]{CA492D}{\textbf{Losing }\textcolor[HTML]{2D4CB9}{Control}: }\textcolor[HTML]{CA492D}{Disruptive }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{2D4CB9}{members }\textcolor[HTML]{2D4CB9}{can }\textcolor[HTML]{CA492D}{derail }\textcolor[HTML]{8E8572}{the }\textcolor[HTML]{CA492D}{performance.\\}\textcolor[HTML]{BBB1A4}{- }\textcolor[HTML]{CA492D}{\textbf{Forcing }\textcolor[HTML]{2D4CB9}{It}: }\textcolor[HTML]{9B60AA}{Unnatural }\textcolor[HTML]{2B4239}{interactions }\textcolor[HTML]{CA492D}{feel }\textcolor[HTML]{2D4CB9}{awkward }\textcolor[HTML]{2D4CB9}{and }\textcolor[HTML]{9B60AA}{contrived.\\}\textcolor[HTML]{9B60AA}{\\}\textcolor[HTML]{9B60AA}{\#\#\# }\textcolor[HTML]{9B60AA}{\textbf{Great }\textcolor[HTML]{9B60AA}{Examples}\\}\textcolor[HTML]{9B60AA}{- }\textcolor[HTML]{9B60AA}{\textbf{Dave }\textcolor[HTML]{BBB1A4}{Chappelle}: }\textcolor[HTML]{9B60AA}{Masters }\textcolor[HTML]{9B60AA}{crowd }\textcolor[HTML]{9B60AA}{work }\textcolor[HTML]{9B60AA}{with }\textcolor[HTML]{9B60AA}{charm }\textcolor[HTML]{9B60AA}{and }\textcolor[HTML]{9B60AA}{wit.\\}\textcolor[HTML]{2B4239}{- }\textcolor[HTML]{2B4239}{\textbf{Jerry }\textcolor[HTML]{BBB1A4}{Seinfeld}: }\textcolor[HTML]{9B60AA}{Uses }\textcolor[HTML]{2B4239}{subtle, }\textcolor[HTML]{2B4239}{observational }\textcolor[HTML]{2B4239}{interactions }\textcolor[HTML]{2B4239}{seamlessly.\\}\textcolor[HTML]{2B4239}{- }\textcolor[HTML]{2B4239}{\textbf{Hannah }\textcolor[HTML]{2D4CB9}{Gadsby}: }\textcolor[HTML]{2B4239}{Deepens }\textcolor[HTML]{BBB1A4}{emotional }\textcolor[HTML]{2D4CB9}{impact }\textcolor[HTML]{2D4CB9}{through }\textcolor[HTML]{2D4CB9}{audience }\textcolor[HTML]{2D4CB9}{engagement.\\}\textcolor[HTML]{2D4CB9}{\\}\textcolor[HTML]{BBB1A4}{\#\#\# }\textcolor[HTML]{CA492D}{\textbf{Conclusion}\\}\textcolor[HTML]{CA492D}{When }\textcolor[HTML]{CA492D}{done }\textcolor[HTML]{CA492D}{well, }\textcolor[HTML]{CA492D}{audience }\textcolor[HTML]{CA492D}{interaction }\textcolor[HTML]{CA492D}{is }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{vital }\textcolor[HTML]{2D4CB9}{tool }\textcolor[HTML]{CA492D}{that }\textcolor[HTML]{CA492D}{elevates }\textcolor[HTML]{2B4239}{a }\textcolor[HTML]{2B4239}{comedian’s }\textcolor[HTML]{CA492D}{delivery, }\textcolor[HTML]{CA492D}{strengthens }\textcolor[HTML]{CA492D}{their }\textcolor[HTML]{CA492D}{stage }\textcolor[HTML]{CA492D}{presence, }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{creates }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{BBB1A4}{memorable, }\textcolor[HTML]{9B60AA}{shared }\textcolor[HTML]{2D4CB9}{experience. }\textcolor[HTML]{2D4CB9}{It }\textcolor[HTML]{8E8572}{requires }\textcolor[HTML]{BBB1A4}{practice, }\textcolor[HTML]{BBB1A4}{sensitivity, }\textcolor[HTML]{CA492D}{and }\textcolor[HTML]{CA492D}{a }\textcolor[HTML]{CA492D}{good }\textcolor[HTML]{CA492D}{read }\textcolor[HTML]{CA492D}{of }\textcolor[HTML]{2D4CB9}{the }\textcolor[HTML]{CA492D}{room, }\textcolor[HTML]{CA492D}{but }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{rewards }\textcolor[HTML]{CA492D}{are }\textcolor[HTML]{CA492D}{well }\textcolor[HTML]{CA492D}{worth }\textcolor[HTML]{CA492D}{the }\textcolor[HTML]{CA492D}{effort.\\}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

